Interpolation-Prediction Networks for Irregularly Sampled Time Series

In this paper, we present a new deep learning architecture for addressing the problem of supervised learning with sparse and irregularly sampled multivariate time series. The architecture is based on the use of a semi-parametric interpolation network followed by the application of a prediction network. The interpolation network allows for information to be shared across multiple dimensions of a multivariate time series during the interpolation stage, while any standard deep learning model can be used for the prediction network. This work is motivated by the analysis of physiological time series data in electronic health records, which are sparse, irregularly sampled, and multivariate. We investigate the performance of this architecture on both classification and regression tasks, showing that our approach outperforms a range of baseline and recently proposed models.

==> model.tex <==
%!TEX root = iclr2019_conference.tex

\section{Model Framework}

In this section, we present the proposed modeling framework. We begin by presenting notation, 
followed by the model architecture and learning criteria.

\subsection{Notation}

We let $\mathcal{D}=\{(\mbf{s}_i,y_i)|i=1,...,N\}$ represent a data set containing
$N$ data cases. An individual data case consists of
a single target value $y_n$ (discrete in the case of classification
and real-valued in the case of regression), as well as a $D$-dimensional, sparse and irregularly
sampled multivariate time series $\mbf{s}_n$. Different dimensions $d$ of the multivariate
time series can have observations at different times, as well as different total
numbers of observations $L_{dn}$. Thus, we represent time series $d$ for data case $n$ as a tuple
$\mbf{s}_{dn}=(\mbf{t}_{dn}, \mbf{x}_{dn})$  where $\mbf{t}_{dn}=[t_{1dn},...,t_{L_{dn}dn}]$
is the list of time points at which observations are defined and 
$\mbf{x}_{dn}=[x_{1dn},...,x_{L_{dn}dn}]$ is the corresponding list of observed values.
\cut{
We represent the time series data with $d$ variables of length $T$ as ${X} = \{\vect{x}_1, \vect{x}_2, \cdots, \vect{x}_T\}^T \in \mathbb{R}^{T*d}$ where $\vect{x}_t \in \mathbb{R}^d$ represents the measurements of all variables recorded at time $t$ and $x_t^j$ represents the value of $j$th variable at time $t$ . 
\begin{equation}
  x_t^j=\begin{cases}
    x_t^j, & \text{if } x_t^j \text{ is recorded.}\\
    0, & \text{otherwise}.
  \end{cases}
\end{equation}


We use masking vector $m_t \in \{0,1\}^d$ to represent  which variables were measured at time $t$. 

\begin{equation}
  m_t^j=\begin{cases}
    1, & \text{if } x_t^j \text{ is observed.}\\
    0, & \text{otherwise}.
  \end{cases}
\end{equation}

We introduce another variable $\vect{z}$ to store the timestamps of the recorded variables. $\vect{z}$ is union of all the recorded timestamps of the $d$ variables for a particular example. We note that the length $\vect{z}$ can vary across the examples. In this work, we are interested in mortality prediction problem on irregularly sampled time series data. We represent the given time series as $\{{X}_n,\vect{z}_n, M_n, l_n \}_{n=1}^N$ where ${X}_n = \{\vect{x}_1^n, \vect{x}_2^n, \cdots, \vect{x}_{T_n}^n\}^T, \vect{z}_n = \{z_1^n, \cdots, z_{T_n}^n\}, {M}_n = \{\vect{m}_1^n, \vect{m}_2^n, \cdots, \vect{m}_{T_n}^n\}^T $ and $l_n \in \{0,1\}.$ 
}
\subsection{Model Architecture}

The overall model architecture consists of two main components: an interpolation
network and a prediction network. The interpolation network interpolates
the multivariate, sparse, and irregularly sampled input time series against 
a set of reference time points $\mbf{r}=[r_1,...,r_T]$. We assume that all of the 
time series are defined within a common time interval (for example, the first 24 or 48  
hours after admission for MIMIC-III dataset). The $T$ reference time points $r_t$ are chosen to be evenly 
spaced within that interval. In this work, we propose a two-layer interpolation network with each layer performing a different type of interpolation.

The second component, the prediction network, takes the output of the interpolation
network as its input and produces a prediction $\hat{y}_n$ for the target variable.
The prediction network can consist of any standard supervised 
neural network architecture (fully-connected feedforward, convolutional, recurrent, etc).
Thus, the architecture is fully modular with respect to the use of different prediction
networks. In order to train the interpolation network, the architecture also includes
an auto-encoding component to provide an unsupervised learning signal in addition to
the supervised learning signal from the prediction network. Figure \ref{fig:model} shows the architecture of the proposed model. We describe the components
of the model in detail below. 

\begin{figure}[h]
\includegraphics[width=0.8\linewidth]{figures/final_model.pdf}
\centering
\caption{Architecture of the proposed model}
\label{fig:model}
\end{figure}
\subsubsection{Interpolation Network} We begin by describing the interpolation network. 
The goal of the interpolation network is to provide a collection of interpolants 
of each of the $D$ dimensions of an input multivariate time series defined at the 
$T$ reference time points $\mbf{r}=[r_1,...,r_T]$. In this work, we use a total
of two interpolation layers and $C=3$ outputs for each of the 
$D$ input time series. The three outputs (discussed in detail below) capture long-term trends, transients, and frequency information. We refer to the interpolation network mapping as the function
$\hat{\mathbf{s}}_n=f_{\theta}(\mbf{s}_n)$ where the dimensions of $\hat{\mathbf{s}}_n$ is $(DC)\times T$.

The first interpolation layer in the interpolation network performs a semi-parametric 
univariate interpolation for each of the $D$ time series separately. The interpolation
is based on a radial basis function network. This
results in a set of values $\hat{x}^{1c}_{kdn}$ for each data case $n$, each input
time series $d$, and each reference time point $r_k$, and each interpolation channel 
$c$ as shown in Equation \ref{eq:interp1}.
\vspace{-1mm}
\begin{align}
 \label{eq:interp1}
{ \hat{x}^{1c}_{kdn} = f^{1c}_{\theta}(r_k,\mbf{s}_n) = \frac{\displaystyle \sum_{j=1}^{L_{dn}} w_{dc}(r_k,t_{jdn}) \:x_{jdn} }{\displaystyle \sum_{j=1}^{L_{dn}}  w_{dc}(r_k,t_{jdn})} } \: , &&
  w_{dc}(r_k,t_{jdn}) = \exp\left(-\alpha_{dc} ||r_k - t_{jdn}||^2\right)
\end{align}

The second interpolation layer merges information from across all of the $D$
time series at each reference time point by taking into account
learnable correlations $\rho_{dd'}$ from across all time series. This
results in a set of values $\hat{x}^{2c}_{kdn}$ for each data case $n$, each input
time series $d$, each reference time point $r_k$, and each interpolation channel 
$c$ as shown in Equation \ref{eq:interp2}. Here, the terms $i_{kdn}$ represent
the intensity of the observations on input dimension $d$ for data  case $n$. The more 
observations that occur near reference time point $r_k$, the larger the value
of $i_{kdn}$. This final interpolation layer thus models the interpolant $\hat{x}^{2c}_{kdn}$ as a weighted linear combination of the
first layer interpolants, while focusing the combination on the time series
$d'$ for which data are actually available at nearby time points.
\vspace{-1mm}
\begin{align}
 \label{eq:interp2}
 \hat{x}^{2c}_{kdn} = f^{2c}_{\theta}(r_k,\mbf{s}_n) =\frac{\sum_{d'} \rho_{dd'} \: i_{kd'n}^c \: \hat{x}^{1c}_{kd'n}}{\sum_{d'} i_{kd'n}^c} \: , &&
 i_{kdn}^c =  f^{3c}_{\theta}(r_k,\mbf{s}_n) = \sum_j w_{dc}(r_k, t_{jdn}) 
\end{align}

In the experiments presented in the next section, we use a total of three
interpolation outputs corresponding to a smooth interpolant to capture
trends, a non-smooth interpolant to capture transients, and the 
intensity function to retain information about where observations occur.
The smooth interpolant corresponds to the first interpolant 
$\hat{\mbf{x}}^{21}_{dn} = [\hat{x}^{21}_{1dn},...,\hat{x}^{21}_{Tdn}]$ \footnote{$\hat{x}^{lc}_{kdn}$ denotes the output of interpolation layer $l$ ($\in \{1,2\}$), and interpolation channel $c$ ($\in \{1,2\}$)for each data case $n$, each input
time series $d$, and each reference time point $r_k$. \label{footnote}}. 
The collection of model parameters associated with this interpolant are the 
cross-dimension correlation coefficients $\rho_{dd'}$, and the 
RBF network bandwidths $\alpha_{d1}$ for all $d$ and $d'$. 

For the non-smooth (transient) interpolant, we start with a second interpolant
$\hat{\mbf{x}}^{12}_{dn} = [\hat{x}^{12}_{1dn},...,\hat{x}^{12}_{Tdn}]$.
The collection of model parameters associated with this 
interpolant are the RBF network parameters $\alpha_{d2}$ for all $d$. 
To accomplish the goal of having this component represent a less smooth interpolation
than  $\hat{\mbf{x}}^{21}_{dn}$, we enforce the relationship 
$\alpha_{d2} = \kappa \alpha_{d1}$ for all $d$ for a value of $\kappa$ greater than one.
This ensures that the temporal similarity decays faster for the component intended to
model transients. To further minimize any redundancy between 
smooth ($\hat{\mbf{x}}^{21}_{dn}$) and non-smooth ($\hat{\mbf{x}}^{12}_{dn}$) component, we subtract the 
smooth interpolant from the non-smooth interpolant leaving the non-smooth
residual: $\hat{\mbf{x}}'^{12}_{dn}=\hat{\mbf{x}}^{12}_{dn}-\hat{\mbf{x}}^{21}_{dn}$ \footref{footnote}.

Finally, for the intensity function, we use 
$\mbf{i}_{dn}^1 = [i^{1}_{1dn},...,i^{1}_{Tdn}]$ (Eq \ref{eq:interp2}). This component 
shares its RBF network parameters \footnote{For the interpolation network, trainable parameters are $\alpha_{d1}$ and $\rho_{dd'}$.} with  $\hat{\mbf{x}}^{21}_{dn}$.
In the experiments, we study the end-to-end impact of each
of these interpolation outputs. 

\subsubsection{Prediction Network} Following the application of the 
interpolation network, all $D$ dimensions of the input multivariate time series have been
re-represented in terms of $C$ outputs defined on the regularly spaced 
set of reference time points $r_1,...,r_T$ (again, in our
experiments, we use $C=3$ as described in the previous section).
Again, we refer to the complete set of interpolation network outputs 
as $\hat{\mathbf{s}}_{n}=f_{\theta}(\mbf{s}_n)$, which can be represented as a matrix
of size $(DC)\times T$. 

The prediction network must take $\hat{\mathbf{s}}_{n}$ as input and
output a prediction $\hat{y}_n=g_{\phi}(\hat{\mbf{s}}_n)=
g_{\phi}(f_{\theta}(\mbf{s}_n))$ of the target value $y_n$
for data case $n$. There are many possible choices for this
component of the model. For example, the matrix $\hat{\mathbf{s}}_{n}$ 
can be converted into a single long vector and provided as 
input to a standard multi-layer feedforward network. 
A temporal convolutional model or a recurrent model like a 
GRU or LSTM can instead be applied to time slices of the 
matrix $\hat{\mathbf{s}}_{n}$. In this work, we conduct experiments
leveraging a GRU network as the prediction network.

\subsubsection{Learning} To learn the model parameters, we use a 
composite objective function consisting of a supervised component
and an unsupervised component. This is due to the fact that the 
supervised component alone is insufficient to learn reasonable
parameters for the interpolation network parameters given the amount
of available training data. The unsupervised component used 
corresponds to an autoencoder-like loss function. However,
the semi-parametric RBF interpolation layers have the ability to
exactly fit the input points by setting the RBF kernel parameters
to very large values. 

To avoid this solution and force the interpolation
layers to learn to properly interpolate the input data, it is necessary
to hold out some observed data points $x_{jdn}$ during learning and then
to compute the reconstruction loss only for these data points. This is a 
well-known problem with high-capacity autoencoders, and past work 
has used similar strategies to avoid the problem of trivially 
memorizing the input data without learning useful structure.

To implement the autoencoder component of the loss, we introduce
a set of masking variables $m_{jdn}$ for each data point $(t_{jdn}, x_{jdn})$.
If $m_{jdn}=1$, then we remove the data point $(t_{jdn}, x_{jdn})$ as an input
to the interpolation network, and include the predicted value of this time point
when assessing the autoencoder loss. We use the shorthand notation $\mbf{m}_n \odot \mbf{s}_n$ to represent
the subset of values of $\mbf{s}_n$ that are masked out, and $(1-\mbf{m}_n) \odot \mbf{s}_n$
to represent the subset of values of $\mbf{s}_n$ that are not masked out. 
The value $\hat{x}_{jdn}$ that we predict for a masked input at time  
point $t_{jdn}$ is the value of the smooth interpolant at that time point, calculated
based on the un-masked input values: $\hat{x}_{jdn} = f^{21}(t_{jdn}, (1-\mbf{m}_n) \odot \mbf{s}_n)$.

Using these definitions, we can now define the learning problem for
the proposed framework. We let $\ell_P$ be the loss for the prediction
network (we use cross-entropy loss for classification and squared 
error for regression). We let $\ell_I$ be the interpolation network autoencoder loss (we use standard squared error).
We also include $\ell_2$ regularizers for both the interpolation
and prediction networks parameters.
%\begin{align}
%	\theta_*,\phi_* &=\argmin_{\theta,\phi} \sum_{n=1}^N \ell_P(y_n, g_{\phi}(f_{\theta}(\mbf{s}_n))\\
%	%
%\nonumber 	&\;\;\;\;\;\;\;\;\;\;\;\;+ \delta \sum_{n=1}^N \sum_{d=1}^D \sum_{j=1}^{L_{dn}} m_{jdn} \ell_I(x_{jdn},f^{21}(t_{jdn}, (1-\mbf{m}_n) \odot \mbf{s}_n))\\
%%
%\nonumber 	&\;\;\;\;\;\;\;\;\;\;\;\;+\lambda_I \Vert \theta \Vert_2^2 + \lambda_P \Vert \phi \Vert_2^2
%\end{align}
\vspace{-4mm}
\begin{align}
	\theta_*,\phi_* &=\argmin_{\theta,\phi} \sum_{n=1}^N \ell_P(y_n, g_{\phi}(f_{\theta}(\mbf{s}_n))
	+ \lambda_I \Vert \theta \Vert_2^2 + \lambda_P \Vert \phi \Vert_2^2 \\
	% 
	\nonumber &\;\;\;\;\;\;\;\;\;\;\;\;+ \delta \sum_{n=1}^N \sum_{d=1}^D \sum_{j=1}^{L_{dn}} m_{jdn} \ell_I(x_{jdn},f^{21}(t_{jdn}, (1-\mbf{m}_n) \odot \mbf{s}_n))
\end{align}
\cut{
\subsubsection{Implementation Details}
The model is learned using the Adam optimization method 
in TensorFlow with gradients provided via automatic differentiation.
However, the actual multivariate time series  
representation used during learning is based on the union
of all time stamps that exist in any dimension of the input time series.
Undefined observations are represented as zeros and a separate
missing data mask is used to keep track of which time series have
observations at each time point. Equations 1 \& 2 are modified such
that data that are not available are not taken into account at all.
This implementation is exactly equivalent to the computations
described in Equations 1 \& 2, but support parallel computation
across all dimensions of the time series for a given data case.

Finally, we note that the learning problem can be solved using a
doubly stochastic gradient based on the use of mini batches
combined with re-sampling the artificial missing data masks 
used in the interpolation loss. In practice, we randomly select
$20\%$ of the observed data points to hold out from every input time
series. 
}
  

\cut{

The interpolation layer creates a smooth interpolation of the irregularly sampled time points with missing data over a set of uniformly sampled reference time points. We use a kernel smoother with a bandwidth parameter to generate the interpolations. In order to capture information from the other time series while interpolation, we introduce correlation variables to capture any correlation present across channels (or variables). If the variables are correlated then we could get some information about a missing value if other variables are recorded
around same time. 
Let $\vect{r} = \{r_1, r_2, \cdots, r_p\}$ be the set of reference points, then interpolation model is defined as:


\[ y_{r_i}^c = \frac{\sum_{c'} \rho_{cc'} \: i_{r_i}^{c'} \: \hat{y}_{r_i}^{c'}}{\sum_{c'} i_{r_i}^{c'}} \qquad  \text{ where}	 \qquad
 \hat{y}_{r_i}^c = \frac{\sum_j w_c(r_i,z_j) \:x_{z_j}^c\: m_{z_j}^c}{\sum_j w_c(r_i,z_j) \: m_{z_j}^c} \] 
\[ i_ {r_i}^c =  \sum_j w_c(r_i,z_j) \: m_{z_j}^c 	\qquad  \text{ and}  \qquad
 w_c(r_i,z_j) = \exp(-\alpha_c ||r_i - z_j||^2)\]
 
 
and $x_{z_j}^c$ represents the value of $c^{th}$ variable at timestamp $z_j$, $y_{r_i}^c$ is the smooth interpolation  of $c^{th}$ variable at reference point $r_i$, , $\hat{y}_{r_i}^c$ is the output of the kernel smoother, $\rho_{cc'}$ represents the correlation between different channels  and $\alpha_c$'s are the inverse bandwidth parameters of the kernel smoother. \\

This interpolation layer leverages both the autocorrelation structure of a single time series, as well its cross-correlation with all other time series present in the input. In addition to the smooth interpolation, we introduce intensity ($i_{r_i}^c$) into our model. Intensity represents the uncertainty in the interpolated value at any particular reference point. If a reference point is close to the observed points of a certain variable, intensity value would be higher which indicates that we would be more certain about the interpolated value at that reference point.\\

To capture the transient (high-frequency) component, we reduce the bandwidth of kernel smoother. Transient component is defined as:
 \[ {v}_{r_i}^c = \frac{\sum_j  \exp(-k\alpha_c ||r_i - z_j||^2) \:x_{z_j}^c\: m_{z_j}^c}{\sum_j  \exp(-k\alpha_c ||r_i - z_j||^2) \: m_{z_j}^c} -  y_{r_i}^c\]
where ${v}_{r_i}^c$ represents the transient component, $k$ is a constant factor by which bandwidth is reduced and $y_{r_i}^c$ is the smooth interpolation. The aim of using lower bandwidth is to capture high frequency components (peaks and troughs) present in the time series. We further investigate how important are each of these components and how much useful information they can provide in performing a classification/regression task on the given time series. Section 4.4 presents an analysis about this. \\

For all the experiments, we select reference points to be uniformly separated by 5 minutes. We have reduced the bandwidth to $1/10^{th}$ i.e. $k = 10$ in order to capture the transient component. Figure \ref{fig:model} shows the architecture of our model. First we have an Autoencoder which generates the smooth interpolation, intensity and transients. We manually mask 20\% of the observed data points in each time series before inputting it to the interpolation layer 2. The interpolation layer then generates a smooth interpolation over all the observed points. We define Autoencoder loss as the mean squared error between the auxiliary output and input over the masked data points. We normalize this loss by dividing it with the variance of each channel before taking the mean. This is done in order to account for the scaling variations present across various channels.\\

It should be noted that both the interpolation layers shown in figure \ref{fig:model} share all the parameters. The smooth interpolation along with transients and intensity act as input to the GRU which then learns to model the sequence. We jointly train all the model parameters with Adam optimization method where the objective function is defined as the sum of Autoencoder loss and cross entropy loss between main output and actual output.





We explore Recurrent Neural Networks (RNN) for modeling time series data because their recursive nature allow them to handle variable length sequences intrinsically.  Among the various variants of RNN, we consider Gated Recurrent Units (Chung et al.  2014). Though other variants such as Long Short Term Memory(LSTMs) networks could also be used.  \\

We develop a novel architecture based on Gated Recurrent Units (GRU) to effectively exploit both the past and the future observations of not just 
same channel but also the correlation present between other channels to accurately model the behavior of missing variables in input time series. 
We introduce an interpolation layer to transform the irregularly sampled time points to  a fixed set of
reference points. Since at training, we have the data available for all the time points, we propose to interpolate the missing variable
using not only the past observations but also the future observations. Our model also learns the correlation present between different channels to accurately model the missing variables. 

We employ an Autoencoder to generate a smooth interpolation of the irregularly sampled input time series over a fixed set of reference points. The resulting smooth interpolation of the raw data is then provided to a GRU as input. Since this smooth interpolation is not able to capture momentary variations, we also explicitly represent transients present in the raw time series using a second interpolant with a much shorter temporal bandwidth.  

\begin{figure}[h]
\includegraphics[width=10cm]{figures/model5.pdf}
\centering
\caption{Model Architecture(left) and Autoencoder(right)}
\label{fig:model}
\end{figure}


Figure \ref{fig:model} shows the architecture of the proposed model. The interpolation layer creates a smooth interpolation of the irregularly sampled time points with missing data over a set of uniformly sampled reference time points. We use a kernel smoother with a bandwidth parameter to generate the interpolations. In order to capture information from the other time series while interpolation, we introduce correlation variables to capture any correlation present across channels (or variables). If the variables are correlated then we could get some information about a missing value if other variables are recorded
around same time. 
Let $\vect{r} = \{r_1, r_2, \cdots, r_p\}$ be the set of reference points, then interpolation model is defined as:
\[ y_{r_i}^c = \frac{\sum_{c'} \rho_{cc'} \: i_{r_i}^{c'} \: \hat{y}_{r_i}^{c'}}{\sum_{c'} i_{r_i}^{c'}} \qquad  \text{ where}	 \qquad
 \hat{y}_{r_i}^c = \frac{\sum_j w_c(r_i,z_j) \:x_{z_j}^c\: m_{z_j}^c}{\sum_j w_c(r_i,z_j) \: m_{z_j}^c} \] 
\[ i_ {r_i}^c =  \sum_j w_c(r_i,z_j) \: m_{z_j}^c 	\qquad  \text{ and}  \qquad
 w_c(r_i,z_j) = \exp(-\alpha_c ||r_i - z_j||^2)\]
and $x_{z_j}^c$ represents the value of $c^{th}$ variable at timestamp $z_j$, $y_{r_i}^c$ is the smooth interpolation  of $c^{th}$ variable at reference point $r_i$, , $\hat{y}_{r_i}^c$ is the output of the kernel smoother, $\rho_{cc'}$ represents the correlation between different channels  and $\alpha_c$'s are the inverse bandwidth parameters of the kernel smoother. \\

This interpolation layer leverages both the autocorrelation structure of a single time series, as well its cross-correlation with all other time series present in the input. In addition to the smooth interpolation, we introduce intensity ($i_{r_i}^c$) into our model which represents the uncertainty in the interpolated value at any particular reference point. If a reference point is close to the observed points of a certain variable, intensity value would be higher which indicates that we would be more certain about the interpolated value at that reference point.\\

To capture the transient (high-frequency) component, we reduce the bandwidth of kernel smoother. Transient component is defined as:
 \[ {v}_{r_i}^c = \frac{\sum_j  \exp(-k\alpha_c ||r_i - z_j||^2) \:x_{z_j}^c\: m_{z_j}^c}{\sum_j  \exp(-k\alpha_c ||r_i - z_j||^2) \: m_{z_j}^c} -  y_{r_i}^c\]
where ${v}_{r_i}^c$ represents the transient component, $k$ is a constant factor by which bandwidth is reduced and $y_{r_i}^c$ is the smooth interpolation. The aim of using lower bandwidth is to capture high frequency components (peaks and troughs) present in the time series. We further investigate how important are each of these components and how much useful information they can provide in performing a classification/regression task on the given time series. Section 4.4 presents an analysis about this. \\

For all the experiments, we select reference points to be uniformly separated by 5 minutes. We have reduced the bandwidth to $1/10^{th}$ i.e. $k = 10$ in order to capture the transient component. Figure \ref{fig:model} shows the architecture of our model. First we have an Autoencoder which generates the smooth interpolation, intensity and transients. We manually mask 20\% of the observed data points in each time series before inputting it to the interpolation layer 2. The interpolation layer then generates a smooth signal over all the observed points. We define Autoencoder loss as the mean squared error between the auxiliary output and input over the masked data points. We normalize this loss by dividing it with the variance of each channel before taking the mean. This is done in order to account for the scaling variations present across various channels.\\

It should be noted that both the interpolation layers shown in figure \ref{fig:model} share all the parameters. The smooth interpolation along with transients and intensity act as input to the GRU which then learns to model the sequence. We jointly train all the model parameters with Adam optimization method where the objective function is defined as the sum of Autoencoder loss and cross entropy loss between main output and actual output.

}
